Machine Learning Systems for Highly-Distributed and Rapidly-Growing Data

The usability and practicality of any machine learning (ML) applications are largely influenced by two critical but hard-to-attain factors: low latency and low cost. Unfortunately, achieving low latency and low cost is very challenging when ML depends on real-world data that are highly distributed and rapidly growing (e.g., data collected by mobile phones and video cameras all over the world). Such real-world data pose many challenges in communication and computation. For example, when training data are distributed across data centers that span multiple continents, communication among data centers can easily overwhelm the limited wide-area network bandwidth, leading to prohibitively high latency and high cost. In this dissertation, we demonstrate that the latency and cost of ML on highly-distributed and rapidly-growing data can be improved by one to two orders of magnitude by designing ML systems that exploit the characteristics of ML algorithms, ML model structures, and ML training/serving data. We support this thesis statement with three contributions. First, we design a system that provides both low-latency and low-cost ML serving (inferencing) over large-scale and continuously-growing datasets, such as videos. Second, we build a system that makes ML training over geo-distributed datasets as fast as training within a single data center. Third, we present a first detailed study and a system-level solution on a fundamental and largely overlooked problem: ML training over non-IID (i.e., not independent and identically distributed) data partitions (e.g., facial images collected by cameras varies according to the demographics of each camera's location).

==> focus/sections/abstract.tex <==
\begin{abstract}

  Large volumes of \kff{video are continuously recorded by} cameras deployed for traffic control and surveillance with the goal of answering ``after the fact'' queries \kff{such as:} {\em identify video frames with objects of certain classes (cars, bags)} from many days of recorded video. %While advancements in convolutional neural networks (\cnns) have enabled answering such queries with high accuracy, they are too expensive and slow.
Current systems for processing such queries on large video datasets incur either high cost at video ingest time or high latency at query time.
We present {\focus}, a system providing both low-cost and low-latency querying on large video datasets. {\focus}' architecture
flexibly and effectively divides the query processing work between \emph{ingest time} and \emph{query time}.
%{\focus} uses cheap ingestion techniques to index the videos by the objects occurring in them. At ingest-time, it uses compressed and specialized \cnns that are cheap. {\focus} handles the lower accuracy of the cheap \cnns by judiciously leveraging expensive \cnns at query-time.
At ingest time (on live videos), {\focus} uses cheap convolutional network classifiers (\cnns) to construct an \emph{approximate index} of all possible object classes in each frame (to handle queries for {\em any} class in the future). At query time, {\focus} leverages this approximate index to provide low latency, but compensates for the lower accuracy of the cheap \cnns through
the judicious use of an expensive \cnn. %, and thus deliver results that are highly accurate at a significantly lower latency. 
%To further reduce query latency, we cluster similar objects and hence avoid redundant processing.
%{\focus}'s architecture allows for smart policies for dividing work between ingest and query stages resulting in orders-of-magnitude faster queries with only a small investment at ingest time. 
%{\focus}'s split architecture enables orders-of-magnitude faster queries with only a small investment at ingest time, and allows flexibly trading off ingest cost and query latency. 
Experiments on commercial video streams %from traffic, surveillance, and news channels, 
show that {\focus}
% smart {\em policies} for dividing work between ingest and query stages leads to it being
is $48\times$ (up to $92\times$) cheaper than using expensive \cnns for ingestion, and
provides $125\times$ (up to $607\times$) lower query latency than a state-of-the-art
video querying system (\sys{NoScope}).

  %{\focus} is also $1.8\times-200\times$ faster than the recently published \sys{NoScope} system\ignore{~\cite{DBLP:journals/pvldb/KangEABZ17}} for video queries.

\end{abstract}


==> focus/sections/acknowledgments.tex <==
\section*{Acknowledgments}

\kff{We thank our shepherd, Andrew Warfield, and the anonymous OSDI reviewers for their valuable and constructive suggestions. We acknowledge the support of our industrial partners: Google, Huawei, Intel, Microsoft, and VMware. This work is supported in part by NSF and Intel STC on Visual Cloud Systems (ISTC-VCS).}


==> focus/sections/related.tex <==
\section{Related Work}
\label{sec:related}

%To our best knowledge, {\focus} is the first system that indexes video and trades off ingest-time cost against query latency for high-accuracy video queries.
%To our best knowledge, {\focus} is the first system that offers low-cost and low-latency CNN-based object detection in videos by balancing between ingest-time cost and query latency.

To our knowledge, {\focus} is the first system that offers low-cost and low-latency queries \kff{for} CNN-based object detection in videos by effectively splitting query-processing work between ingest time and query time. % ingest-time cost and query latency.
%To our best knowledge, {\focus} is the first system that balances ingest-time cost against query latency for video datasets to deliver high accuracy results. % system to balance the potentially wasted ingest cost against query latency on large video datasets by (1) \emph{approximately} indexing video streams at ingest time using compressed and specialized \cnn models, (2) reducing query latency by clustering similar objects using \cnn feature vectors, and (3) judiciously leveraging expensive \cnn models at query time to deliver high precision results.
We \kff{discuss key
works} related to our system.%: 1) cascaded classification, 2) \cnn compression, 3) context-specific model specialization, and 4) stream processing systems.%, all of which are related to our proposed system.

\noindent{\bf 1) Cascaded classification.}
Various works in vision research propose speeding up classification by cascading a
series of classifiers. Viola et al.~\cite{DBLP:conf/cvpr/ViolaJ01} is the earliest work \kff{that}
cascades a series of classifiers (from the simplest to the most
complicated) to quickly disregard regions in an image. Many improvements follow (e.g., ~\cite{DBLP:conf/icip/LienhartM02,
  DBLP:journals/tkde/YangLCP06, DBLP:conf/icml/XuKWC13}). \cnns are also cascaded (e.g.,
~\cite{DBLP:conf/cvpr/SunWT13, DBLP:conf/cvpr/LiLSBH15, mcdnn,
  DBLP:conf/iccv/CaiSV15}) to reduce object
detection latency. %At a high level, our work bears some resemblance to this idea, but we are different in two major ways.
Our work is different in two major ways. First, we \emph{decouple} the compressed
\cnn from the GT-CNN, which enables us to choose from a wider range of
ingest-time \cnns and \kff{thus} enables better trade-offs
between ingest cost and query latency, a key aspect of our
work. Second, we cluster similar objects using \cnn features to
eliminate redundant work, which is an effective
technique for video streams.

\ignore{
\noindent{\bf 2) Neural network compression.}
Recent work proposes various
techniques to reduce the running time of \cnns. These techniques include shallow
models~\cite{DBLP:conf/nips/BaC14}, predicting
weights~\cite{DBLP:conf/nips/DenilSDRF13}, matrix
pruning~\cite{pruning1,pruning2}, model quantization~\cite{DBLP:conf/iclr/HanMD16}, and others
(e.g.,~\cite{lowrank, fitnets, DBLP:conf/nips/DentonZBLF14,
  DBLP:conf/sips/HwangS14, DBLP:conf/icassp/AnwarHS15,
  DBLP:journals/corr/HintonVD15, DBLP:conf/eccv/RastegariORF16}). %Most of these efforts reduce resource consumption at the expense of accuracy.
Our work is largely orthogonal to these, in that our system
is not tied to a specific model compression technique, and we can
employ any of these techniques. \ga{Nix this paragraph to save space.}% to provide more flexibility.
}

\noindent{\bf 2) Context-specific model specialization.}
%Another approach to improve the performance of \cnns is context-specific model specialization. %The idea is that a specific scene or task usually has highly skewed data distribution, so a
Context-specific specialization of models can improve
accuracy~\cite{DBLP:conf/dicta/MhallaMCGA16} or \kff{speed up inference}~\cite{mcdnn, DBLP:journals/pvldb/KangEABZ17,
  DBLP:journals/corr/ShenHPK17}. Among these, the closest to our work
is NoScope~\cite{DBLP:journals/pvldb/KangEABZ17}. 
%\kv{\sys{NoScope} optimizes \cnns for a single class, and applies all the optimization at query time. In contrast, {\focus} splits the work between ingest- and query-time, and its ingest processing can handle all classes. These architectural differences make {\focus} much more effective than \sys{NoScope}, especially for querying complicated videos, achieving high recall/precision targets, and for less frequent object classes.}
\gaa{\sys{NoScope} optimizes for the specified class at query-time using lightweight binary classifiers. In contrast, {\focus}' architecture splits work between ingest and query times, leading to two orders of magnitude lower latency (\xref{sec:evaluation}). To achieve these gains, \kff{{\focus} uses} techniques to index {\em all possible classes} at ingest-time, and thus can handle any class that will get queried in the future. {\focus}' indexing is especially effective for \kff{less frequent} object classes, which is arguably of more interest for video querying systems.}

%, which aims to optimize \cnn-based video queries. A few key differences stand out. 
%First, NoScope applies all the optimizations at query-time, while {\focus} adopts a different architecture by splitting work between ingest- and query-time. Thus, {\focus} trades off higher ingest cost for {\em even lower} query latency.
%Second, NoScope optimizes \cnns for a single class, while we optimize ingest \cnns for all frequent classes in the stream and allow queries even for the rare -- OTHER -- classes. 
%Finally, we use the object feature vectors to cluster similar objects and create an index to map classes to clusters; this allows us to efficiently query across {\em all} classes, while NoScope has to redo all query-time work, including training specialized CNNs, for each query.

%Unlike {\focus}, NoScope does not split work between ingest-time and query-time; it applies all the optimizations at query-time. Hence, they do not have to deal with the balancing that {\focus} has to do between ingest-time and query-time costs.
%Further, they optimize for a specific object class to be queried per stream while we index for all the classes. Finally, NoScope employs pixel-level differencing to eliminate redundancy, while our technique of clustering using feature vectors is more robust as per our experiments.

%NoScope employs pixel-level difference
%detector to eliminate redundant frames and a \emph{query-specific}
%binary classifier to short-circuit \cnn evaluation. In contrast, our
%work tackles a different and more general problem, as we \emph{do not}
%assume which class would be queried at ingest time. Thus, our
%ingest-time top-{\sf K} indexing helps queries on \emph{all} classes,
%and our system is complementary to query-time optimizations such as
%binary classifiers.% to further improve query latency.

\noindent{\bf 3) Stream processing systems.}
Systems for general stream data processing (e.g.,~\cite{DBLP:conf/cidr/AbadiABCCHLMRRTXZ05, amini2006spc,
  DBLP:conf/sigmod/ChandrasekaranCDFHHKMRS03,
  DBLP:conf/vldb/CarneyCCCLSSTZ02, storm, DBLP:conf/vldb/TatbulCZ07,
  DBLP:conf/vldb/TuLPY06, DBLP:conf/sosp/ZahariaDLHSS13,
  DBLP:conf/nsdi/RabkinASPF14, DBLP:conf/nsdi/LinFQXYZZ16,
  DBLP:conf/sigmod/BailisGMNRS17}) 
and specific to video \kff{stream} analytics
(e.g.,~\cite{DBLP:conf/nsdi/ZhangABPBF17}) %or network monitoring (e.g.,~\cite{DBLP:conf/sigmod/CranorJSS03}). These efforts
mainly
focus on general stream processing challenges such as load
shedding, fault tolerance, distributed execution, or limited network
bandwidth. In contrast, our work is specific to querying on recorded video
data with ingest and query trade-offs, \kff{and, thus, mostly orthogonal}.
{\focus} coud be integrated with one of these general stream
processing systems. \ignore{to build a more fault tolerant system.}

\noindent{\bf 4) Video indexing and retrieval.} A large body of work
in multimedia and information retrieval research proposes various
content-based video indexing and retrieval techniques to facilitate
queries on videos (e.g., ~\cite{DBLP:journals/mta/SnoekW05,
  DBLP:journals/tomccap/LewSDJ06, DBLP:journals/ftir/SnoekW09,
  DBLP:journals/tsmc/HuXLZM11}). Among them, most works focus on
indexing videos for different types of queries, such as shot boundary
detection (e.g.,~\cite{DBLP:journals/tcsv/YuanWXZLLZ07}), semantic
video search (e.g.,~\cite{DBLP:journals/sigmod/Hampapur99,
  DBLP:journals/tip/DagtasAGK00, DBLP:conf/icassp/ChangMS07}), video
classification (e.g.,~\cite{DBLP:journals/tsmc/BrezealeC08}),
spatio-temporal information-based video retrieval
(e.g.,~\cite{DBLP:journals/pr/RenSSZ09,
  DBLP:journals/vldb/DonderlerUG04}) or subsequence similarity search
(e.g.,~\cite{DBLP:conf/sigmod/ShenZH05,
  DBLP:journals/vldb/ZhouZCB12}). Some works
(e.g.,~\cite{DBLP:conf/civr/ChristelC06,
  DBLP:conf/trecvid/SnoekSRHGORGWKS10}) focus on the query interface
to enable \kff{querying} by keywords, concepts, or examples. \kv{These works are
largely orthogonal to our work because we focus on reducing \emph{cost and
  latency} of \cnn-based video queries, not on creating an indexing structure for new query
types or query interfaces. We believe our approach of splitting
ingest-time and query-time work can
be extended to many different types of video queries (\xref{sec:other_use}).}

\noindent\kv{{\bf 5) Database indexing.} Using index structures to reduce query latency~\cite{DBLP:books/daglib/0015084} is a commonly-used technique in conventional databases (e.g.,~\cite{DBLP:conf/sigmod/BayerM70, DBLP:journals/tods/LehmanY81}), key-value databases (e.g.,~\cite{DBLP:conf/eurosys/MaoKM12}), similarity search (e.g.,~\cite{DBLP:conf/sigmod/Guttman84, DBLP:conf/vldb/GionisIM99}), graph queries (e.g.,~\cite{DBLP:journals/vldb/YuanM13}), \kff{genome analysis (e.g.,~\cite{alkan2009personalized, DBLP:journals/bmcgenomics/XinLHYMA13})}, and many others. \kf{Our \sys{Ingest-heavy} and \sys{Ingest-NoScope} baselines are also examples that index all video frames at ingest time. While queries are naturally faster with these baselines, they are too costly and are potentially wasteful for large-scale videos}. In contrast, our work offers new trade-off options between ingest cost and query latency by creating low-cost approximate indexes at ingest time and retaining high accuracy with little work at query time. }

%Indexing is a well-studied technique in database research~\cite{DBLP:books/daglib/0015084}. 
%


==> gaia/sections/abstract.tex <==
\begin{abstract}


Machine learning (ML) is widely used to derive useful information from
large-scale data (such as user activities, pictures, and videos)
generated at increasingly rapid rates, \emph{all over the
  world}. Unfortunately, it is infeasible to move all this
globally-generated data to a centralized data center before running an
ML algorithm over it{\textemdash}moving large amounts of raw data over
\khi{wide-area networks (WANs)} can be extremely slow, and is also
subject to \khii{the constraints of privacy and data sovereignty
  laws}. This motivates the need for a geo-distributed ML system
spanning \emph{multiple data centers}.  Unfortunately, communicating
over WANs can significantly degrade ML system performance (by as much
as 53.7$\times$ in our study) because the communication overwhelms the
limited WAN bandwidth.

Our goal in this work is to develop a \emph{geo-distributed} ML system
that (1) employs an intelligent communication mechanism over WANs to
efficiently utilize the scarce WAN bandwidth, while retaining the
accuracy and correctness guarantees of an ML algorithm; and (2) is
generic and flexible enough to run a wide range of ML algorithms,
without requiring any changes to the algorithms.
%%% ONUR: accuracy and correctness are a bit mouthful.

To this end, we introduce a new, general geo-distributed ML system,
\emph{{\gaia}}, that decouples the communication \emph{within} a data
center from the communication \emph{between} data centers, enabling
different communication and consistency models for each.  We present a
new ML \synchronization model, \emph{\protocol (\protoabbrv)},
\khii{whose key idea is to dynamically eliminate \emph{insignificant}
  communication} between data centers while still guaranteeing the
\khii{correctness} of ML algorithms. Our experiments on our prototypes
of {\gaia} running across 11 Amazon EC2 global regions and on a cluster
that emulates EC2 WAN bandwidth show that {\gaia} provides
1.8--53.5$\times$ \khi{speedup over two state-of-the-art} distributed
ML systems, and is within 0.94--1.40$\times$ of \khi{the speed of
  running the same ML algorithm on machines on a local area network
  (LAN). }

\end{abstract}


==> gaia/sections/acknowledge.tex <==
\section*{Acknowledgments}

\khi{We thank our shepherd, Adam Wierman, and the reviewers for their
  valuable suggestions. We thank the SAFARI group members and Garth
  A. Gibson for their feedback. Special thanks to Henggang Cui for his
  help on IterStore and GeePS, Jinliang Wei for his help on B\"{o}sen,
  and their feedback. We thank the members and companies of the PDL
  Consortium (including Broadcom, Citadel, EMC, Facebook, Google, HP
  Labs, Hitachi, Intel, Microsoft Research, MongoDB, NetApp, Oracle,
  Samsung, Seagate, Tintri, Two Sigma, Uber, Veritas, and Western
  Digital) for their interest, insights, feedback, and support. We
  acknowledge the support of our industrial partners: Google, Intel,
  NVIDIA, Samsung and VMWare. This work is supported in part by NSF
  grant 1409723, Intel STC on Cloud Computing (ISTC-CC), Intel STC on
  Visual Cloud Systems (ISTC-VCS), and the Dept of Defense under
  contract FA8721-05-C-0003. Dimitris Konomis is partially supported
  by Onassis Foundation.}


==> gaia/sections/relatedwork.tex <==
\section{Related Work}

To our knowledge, this is the first work to propose a globally
distributed ML system that \khi{is} (1) designed to run effectively
over WANs while ensuring the \khi{convergence} and accuracy of an ML
algorithm, and (2) generic and flexible to run a wide range of ML
algorithms \khii{\emph{without} requiring modification}. In this
section, we discuss related works on 1) WAN-aware data analytics and
ML systems, 2) distributed ML systems, 3) non-uniform convergence in
ML algorithms, 4) communication-efficient ML algorithms, and 5)
approximate queries on distributed data, all of which are related to
our proposed system.

\textbf{WAN-aware Data Analytics and ML Systems.} Prior work
establishes the emerging problem of analyzing the globally-generated
data in the context of data analytics systems
(e.g.,~\cite{DBLP:conf/nsdi/VulimiriCGJPV15,
  DBLP:conf/nsdi/RabkinASPF14, DBLP:conf/sigcomm/PuABKABS15, clarinet,
  DBLP:conf/hpdc/HeintzCS15, DBLP:conf/cloud/HungGY15,
  DBLP:journals/pvldb/KloudasRPM15,
  DBLP:conf/cidr/VulimiriCGKV15}). These works show very promising WAN
bandwidth reduction and/or system performance improvement with a
WAN-aware data analytics framework. However, their goal is \emph{not}
to run an \emph{ML system} effectively on WANs, which has very
different challenges from a data analytics system. Cano et
al.~\cite{DBLP:journals/corr/CanoWMCF16} first discuss the problem of
running an ML system on \khii{geo-distributed} data. They show that a
geo-distributed ML system can perform significantly better by
leveraging a communication-efficient
algorithm~\cite{DBLP:journals/corr/MahajanKSB13} for logistic
regression models. This solution requires the ML programmer to change
the ML algorithm, which is challenging and algorithm-specific. In
contrast, our work focuses on the design of
\khi{communication-efficient mechanisms at the system level} and
requires no modification to the ML algorithms.

\ignore{ \cite{DBLP:journals/corr/CanoWMCF16} is the only work to
  tackle running an ML system on geographically distributed data. They
  propose a new approach, Geo-Distributed Machine Learning (GDML),
  that leverages a communication-efficient
  algorithm~\cite{DBLP:journals/corr/MahajanKSB13} for logistic
  regression models. This solution, however, is highly specific to a
  certain class of ML algorithms (linear models), and requires the ML
  programmer to alter the algorithm itself to make it WAN
  efficient. Thus, it is important to explore new solutions that are
  \emph{general}, and hence applicable, to a wide variety of ML
  algorithms, without requiring any change to the ML algorithms or
  program.  }

\textbf{Distributed ML Systems.} There are many distributed ML systems
that aim to enable large-scale ML applications (e.g.,~\cite{Mllib,
  Mahout, LowGKBGH12, DBLP:conf/osdi/ChilimbiSAK14, DeanCMCDLMRSTYN12,
  HoCCLKGGGX13, CuiTWXDHHGGGX14, XingHDKWLZXKY15, CuiCHKLKWDGGGX14,
  DBLP:conf/osdi/LiAPSAJLSS14, DBLP:conf/nips/LiASY14,
  DBLP:conf/cloud/WeiDQHCGGGX15, tensorflow2015-whitepaper,
  AhmedAGNS12, DBLP:conf/eurosys/KimHLZDGX16,
  DBLP:conf/eurosys/CuiZGGX16}). These systems successfully
demonstrate their effectiveness \khi{on a} large number of machines by
employing various synchronization models and system
optimizations. However, all of them assume \khi{that} the network
communication happens \emph{within} a data center and do not tackle
the challenges \khii{of} scarce WAN bandwidth. As our study shows,
state-of-the-art parameter server systems suffer from significant
performance degradation and data transfer cost when deployed across
multiple data centers on WANs. We demonstrate our idea on both
CPU-based and GPU-based parameter server
systems~\cite{CuiTWXDHHGGGX14, DBLP:conf/eurosys/CuiZGGX16}, and we
believe our proposed general solution can be applied to all
distributed ML systems that use the parameter server architecture.

\textbf{Non-uniform Convergence in ML Algorithms.} Prior work observes
that, in many ML algorithms, not all model parameters converge to
their optimal value within the same number of computation
iterations~\cite{lars, DBLP:conf/uai/ElidanMK06, LowGKBGH12,
  DBLP:conf/cloud/ZhangGGW11, DBLP:conf/eurosys/KimHLZDGX16}. Several
systems exploit this property to improve the algorithm convergence
\khi{speed, e.g., by} prioritizing the computation of important
parameters~\cite{LowGKBGH12, DBLP:conf/cloud/ZhangGGW11,
  DBLP:conf/eurosys/KimHLZDGX16}, communicating the important
parameters more aggressively~\cite{DBLP:conf/cloud/WeiDQHCGGGX15}, or
sending \khii{fewer} updates with user-defined
filters~\cite{DBLP:conf/osdi/LiAPSAJLSS14, DBLP:conf/nips/LiASY14}.

Among \khi{these}, the closest to our work is Li et al.'s proposal for
a communication-efficient parameter server
system~\cite{DBLP:conf/osdi/LiAPSAJLSS14, DBLP:conf/nips/LiASY14},
which employs various filters to reduce communication between worker
machines and parameter servers. In contrast to our work, this work 1)
does not differentiate the communication on LANs from the
communication on WANs, \khi{and thus it cannot} make efficient use of
the abundant LAN bandwidth or the scarce and heterogeneous WAN
bandwidth, and 2) does not propose a general \synchronization model
across multiple data centers, a key contribution of our work.

\ignore{None of these works exploits this property
to propose a theoretical robust synchronization model across multiple
data centers, which forms a key contribution of our work. As we show
in Section~\ref{subsec:async}, simply sending less updates without
synchronization mechanisms can cause the algorithm to diverge from the
optimum point.}

\textbf{Communication-Efficient ML Algorithms.} A large body of prior
work proposes ML algorithms to reduce the dependency on intensive
parameter updates to enable more efficient parallel computation
(e.g.,~\cite{DBLP:conf/nips/JaggiSTTKHJ14,
  DBLP:journals/jmlr/ZhangDW13, DBLP:conf/nips/ZinkevichWSL10,
  DBLP:conf/icml/TakacBRS13, DBLP:conf/uai/NeiswangerWX14,
  DBLP:conf/icml/ShamirS014, DBLP:conf/icml/ZhangL15a}). These works
are largely orthogonal to our work, as we focus on a generic
system-level solution \khii{that does not require any changes to ML
  algorithms}. These ML algorithms can use our system to further
reduce communication overhead over WANs.

\textbf{Approximate Queries on Distributed Data.} In the database
community, there is substantial prior work that explores the trade-off
between precision and performance for queries on distributed data over
WANs (e.g.,~\cite{DBLP:conf/ssdbm/WolfsonXCJ98,
  DBLP:conf/vldb/OlstonW00, DBLP:conf/sigmod/OlstonJW03,
  DBLP:conf/sigmod/CormodeGMR05}). The idea is to reduce communication
overhead of moving \khi{up-to-date} data from data sources to a query
processor by allowing some user-defined precision loss for the
queries. At a high level, our work bears some resemblance \khi{to}
this idea, but the challenges we tackle are fundamentally
different. The focus of distributed database systems is on
approximating queries (e.g., simple aggregation) on raw data. In
contrast, our work focuses on retaining ML algorithm convergence and
accuracy by using approximate ML models during training.



==> noniid/sections/abstract.tex <==
\begin{abstract}
  Many large-scale machine learning (ML) applications need to train ML models over \emph{decentralized} datasets that are generated at different devices and locations. These decentralized datasets pose a fundamental challenge to ML because they are typically generated in very different contexts, which leads to significant differences in data distribution across devices/locations. In this work, we take a step toward better understanding this challenge, by presenting the first detailed experimental study of the impact of such \emph{non-IID data} on the decentralized training of deep neural networks (DNNs). Our study shows that: (i) the problem of non-IID data partitions is fundamental and pervasive, as it exists in all ML applications, DNN models, training datasets, and decentralized learning algorithms in our study; (ii) this problem is particularly difficult for DNN models with batch normalization layers; and (iii) the degree of deviation from IID (the skewness) is a key determinant of the difficulty level of the problem.  With these findings in mind, we present \sscout, a system-level approach that adapts the communication frequency of decentralized learning algorithms to the (skew-induced) accuracy loss between data partitions.  We also show that group normalization can recover much of the skew-induced accuracy loss of batch normalization.
\end{abstract}

==> noniid/sections/discussion.tex <==
\section{Discussion: Regimes of Non-IID Data}


==> noniid/sections/relatedwork.tex <==
\section{Related Work}

To our knowledge, this is the first detailed study on the problem of non-IID data partitions for decentralized learning. 
Our study shows that this is a fundamental and pervasive problem, and we investigate various aspects of this problem, such as decentralized learning algorithms, batch normalization, and the degree of non-IID data, as well as present our \sscout{} approach.
Here, we discuss related work.

\textbf{Large-scale systems for centralized learning.} 
There are many large-scale ML systems that aim to enable efficient ML training with \emph{centralized} datasets (e.g.,~\cite{DBLP:conf/nips/RechtRWN11, LowGKBGH12, DBLP:conf/osdi/ChilimbiSAK14, DeanCMCDLMRSTYN12, HoCCLKGGGX13, CuiTWXDHHGGGX14, DBLP:conf/osdi/LiAPSAJLSS14, DBLP:journals/corr/ChenLLLWWXXZZ15, DBLP:journals/corr/GoyalDGNWKTJH17}), where the data reside within a single data center. 
Some of them propose communication-efficient designs, such as relaxing synchronization requirements~\cite{DBLP:conf/nips/RechtRWN11, HoCCLKGGGX13, DBLP:journals/corr/GoyalDGNWKTJH17} or sending fewer updates to parameter servers~\cite{DBLP:conf/osdi/LiAPSAJLSS14, DBLP:conf/nips/LiASY14}. 
These works assume the training data are centralized so they can be easily partitioned among the machines performing the training in an IID manner (e.g., by random shuffling). 
Hence, they are neither designed nor validated on non-IID data partitions.

\ignore{
\textbf{Communication-efficient training for specific algorithms.} 
A large body of prior work proposes ML training algorithms to reduce the dependency on intensive parameter updates to enable more efficient parallel training (e.g.,~\cite{DBLP:conf/nips/JaggiSTTKHJ14, DBLP:journals/jmlr/ZhangDW13, DBLP:conf/nips/ZinkevichWSL10, DBLP:conf/icml/TakacBRS13, DBLP:conf/uai/NeiswangerWX14, DBLP:conf/icml/ShamirS014, DBLP:conf/icml/ZhangL15a, DBLP:journals/jmlr/Shalev-Shwartz013}). 
These works reduce communication overhead by proposing algorithm-specific approaches, such as solving a dual problem~\cite{DBLP:journals/jmlr/Shalev-Shwartz013, DBLP:conf/icml/TakacBRS13, DBLP:conf/nips/JaggiSTTKHJ14} or employing a different optimization algorithm~\cite{DBLP:conf/icml/RakhlinSS12, DBLP:conf/icml/ZhangL15a}. 
The main drawback of these approaches is that they are not general and their applicability depends on the ML application. 
Besides, these works also assume centralized, IID data partitions. 
Thus, their effectiveness over decentralized, non-IID data partitions needs much more study.
}

\textbf{Decentralized learning.} 
As most training data are generated in a decentralized manner, prior work proposes communication-efficient algorithms (e.g.,~\cite{DBLP:conf/nsdi/HsiehHVKGGM17, DBLP:conf/aistats/McMahanMRHA17, DBLP:conf/ccs/ShokriS15, DBLP:conf/ICLR/LinHMWD18, DBLP:conf/icml/TangLYZL18}) for ML training over decentralized datasets. 
%Among them, the most common settings are federated learning~\cite{DBLP:conf/aistats/McMahanMRHA17} and geo-distributed learning~\cite{DBLP:conf/nsdi/HsiehHVKGGM17}. 
However, the major focus of these works is to reduce communication overhead among data partitions, and they either \emph{(i)} assume the data partitions are IID~\cite{DBLP:conf/nsdi/HsiehHVKGGM17, DBLP:conf/ccs/ShokriS15, DBLP:conf/ICLR/LinHMWD18} or \emph{(ii)} conduct only a limited study on non-IID data partitions~\cite{DBLP:conf/aistats/McMahanMRHA17, DBLP:conf/icml/TangLYZL18}. 
As our study shows, these decentralized learning algorithms lose significant model quality in the Non-IID setting (\xref{sec:overview}). 
Some recent work~\cite{DBLP:journals/corr/abs-1806-00582, DBLP:conf/nips/SmithCST17} investigates the problem of non-IID data partitions. 
For example, instead of training a global model to fit non-IID data partitions, federated multi-task learning~\cite{DBLP:conf/nips/SmithCST17} proposes training local models for each data partition while leveraging other data partitions to improve the model accuracy. 
However, this approach does not solve the problem for global models, which are essential when a local model is unavailable (e.g., a brand new partition without training data) or ineffective (e.g., a partition with too few training examples for a class).
%, such as kangaroos in Europe). 
The closest to our work is Zhao et al.'s study~\cite{DBLP:journals/corr/abs-1806-00582} on \fedavg over non-IID data, which shows \fedavg suffers significant accuracy loss in the Non-IID setting. 
While the result of their study aligns with our observations on \fedavg, our study \emph{(i)} broadens the problem scope to a variety of decentralized learning algorithms, ML applications, DNN models, and datasets, \emph{(ii)} explores the problem of batch normalization and possible solutions, and \emph{(iii)} designs and evaluates \sscout.


==> sections/timeline.tex <==
\section{Goal and Timeline for Graduation}

\begin{table}[H]
\small
\begin{tabular}{p{1.5in} p{4.7in}}  
\toprule
Duration & Description \\ 
\midrule
Aug 2018 & Work on characterization of ML training over skewed data distribution \\
\midrule
Sep 2018 & Work on final version and presentation of {\focus} \\
\midrule
Oct 2018-Jan 2019 & Work on solutions for ML training over skewed data distribution and potentially submit our work to a top systems/ML conference \\
\midrule
Feb-Mar 2019 & Wind up on work and start writing thesis \\
\midrule
April/May 2019 & Defense \\
\toprule
\end{tabular}
\caption{Timeline for the proposal}
\end{table}

